CERNLIB status

We present a revived version of CERNLIB, the basis for software ecosystems of most of the pre-LHC HEP experiments. The efforts to consolidate CERNLIB are part of the activities of the Data Preservation for High Energy Physics collaboration to preserve data and software of the past HEP experiments. The presented version is based on CERNLIB version 2006 with numerous patches made for compatibility with modern compilers and operating systems. The code is available in the CERN GitLab repository with all the development history starting from the early 1990s. The updates also include a re-implementation of the build system in CMake to ensure CERNLIB compliance with the current best practices and to increase the chances of preserving the code in a compilable state for the decades to come. The revived CERNLIB project also includes updated documentation, which we believe is a cornerstone for any preserved software depending on it.

==> Makefile <==
#ulimit -u 10000
latexfile?=CL
newname?=CL
STYLE=proceedings


LATEX=  lualatex -halt-on-error -shell-escape -enable-write18
LATEX=  pdflatex -halt-on-error -shell-escape -enable-write18
BIBTEX=bibtex
UNAME_S := $(shell uname -s)
ifeq ($(UNAME_S),Linux)
SED=sed
endif
ifeq ($(UNAME_S),Darwin)
SED=gsed
endif


figures=Figures/JADE.001.pdf Figures/delgra_2022_ubuntu2.pdf Figures/grope.pdf

latexfiles=  $(latexfile)-txt.tex $(latexfile)-val.tex 
ifeq ($(STYLE),proceedings)
	latexfiles=
	STYLE_SPECIFIC_FILES=$(latexfile)-proceedings.tex jpconf.cls jpconf11.clo  iopart-num.bst
endif


ifeq ($(STYLE),draft)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-draft.tex $(latexfile).bst
endif

ifeq ($(STYLE),arxiv)
	latexfiles=
	STYLE_SPECIFIC_FILES=$(latexfile)-proceedings.tex jpconf.cls jpconf11.clo  iopart-num.bst
endif

ifeq ($(STYLE),epjc)
	STYLE_SPECIFIC_FILES=svjour.cls  svepj.clo $(latexfile)-epjc.tex $(latexfile).bst
endif


all: $(latexfile)-$(STYLE).pdf

tar:  Makefile $(figures) $(constanttables) $(tables)   $(latexfiles) $(STYLE_SPECIFIC_FILES)
	rm -rf TAR
	mkdir -p TAR
	cp Makefile   $(latexfiles)  $(latexfile).bib   $(STYLE_SPECIFIC_FILES) TAR
ifeq ($(STYLE),epjc)
	cp $(figures) TAR/
else
	mkdir -p TAR/Figures
	cp $(figures) TAR/Figures
endif
	$(SED) -i 's@'$(latexfile)'@'$(newname)'@g' TAR/*tex	
	$(SED) -i 's@'$(latexfile)'@'$(newname)'@g' TAR/Makefile
	$(SED) -i 's@^STYLE.*@STYLE='$(STYLE)'@g' TAR/Makefile
	$(SED) -i '/@artic/achecked={2},'     TAR/*bib	
	$(SED) -i '/@inproceed/achecked={2},' TAR/*bib	
	$(SED) -i '/@phdthesis/achecked={2},' TAR/*bib	

ifeq ($(STYLE),epjc)
	$(SED) -i 's@\[htbp\]@@g' TAR/$(latexfile)-tab.tex
	$(SED) -i 's@c|@c@g' TAR/$(latexfile)-tab.tex
	$(SED) -i 's@|c@c@g' TAR/$(latexfile)-tab.tex
	$(SED) -i 's@}|@}@g' TAR/$(latexfile)-tab.tex
endif

ifneq ($(STYLE),proceedings)
	mv TAR/$(latexfile).bst TAR/$(newname).bst 
endif
	mv TAR/$(latexfile).bib TAR/$(newname).bib 
	mv TAR/$(latexfile)-$(STYLE).tex TAR/$(newname)-$(STYLE).tex
ifeq ($(STYLE),epjc)
	$(SED) -i 's@Figures/@@g' TAR/Makefile
endif
ifeq ($(STYLE),proceedings)
	#mv TAR/$(latexfile)-def.tex TAR/$(newname)-def.tex
	#cat TAR/$(latexfile)-val.tex | grep [:0-9:] > TAR/$(newname)-val.tex
	#rm -f  TAR/$(newname)-txt.tex TAR/$(latexfile).bst TAR/$(newname).bst 
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
	#rm -rf TAR/$(newname).bib 
endif
ifeq ($(STYLE),arxiv)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
ifeq ($(STYLE),epjc)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
	tar -zcvf   $(newname).tar.gz -C TAR . 
	rm -rf $(newname).zip; cd TAR; zip ../$(newname).zip ./*/* ./*; cd ..

	rm -rf TAR


tables=
constanttables=


$(latexfile)-$(STYLE).pdf :  $(figures) $(constanttables) $(tables) \
                    $(latexfiles)  $(latexfile).bib  $(STYLE_SPECIFIC_FILES) 
                    #answers.tex
	#$(LATEX) answers.tex
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
ifeq ($(STYLE),epjc)
	$(SED) -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
ifeq ($(STYLE),arxiv)
	$(SED) -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
	$(SED) -i 's@Collaboration@Coll\.@g'  $(latexfile)-$(STYLE).bbl
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)

pdf : $(latexfile)-$(STYLE).pdf

$(latexfile).rws: $(latexfile)-dict.txt
	aspell --lang=en create master ./$(latexfile).rws < ./$(latexfile)-dict.txt

spell: $(latexfile).rws
	for a in $$(ls -1 $(latexfile)-*.tex ); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-extra-dicts=./$(latexfile).rws  -t --dont-tex-check-comments -d en_GB -c $$a ;\
	done

clean :
	rm -f *.aux
	rm -f *.lof
	rm -f *.out
	rm -f *.lot
	rm -f *.bbl
	rm -f *.l4l
	rm -f *.log
	rm -f *.blg
	rm -f *.ilg
	rm -f *.aux
	rm -f $(latexfile)*.dvi
	rm -f $(latexfile)*.ps
	rm -f $(latexfile)*.pdf
	rm -f *.toc
	rm -f *.idx
	rm -f *.ind
	rm -f *.nav
	rm -f *.snm


